Towards Cross-Modal Text-Molecule Retrieval with Better Modality Alignment

Cross-modal text-molecule retrieval model aims to learn a shared feature space of the text and molecule modalities for accurate similarity calculation, which facilitates the rapid screening of molecules with specific properties and activities in drug design. However, previous works have two main defects. First, they are inadequate in capturing modality-shared features considering the significant gap between text sequences and molecule graphs. Second, they mainly rely on contrastive learning and adversarial training for cross-modality alignment, both of which mainly focus on the first-order similarity, ignoring the second-order similarity that can capture more structural information in the embedding space. To address these issues, we propose a novel cross-modal text-molecule retrieval model with two-fold improvements. Specifically, on the top of two modality-specific encoders, we stack a memory bank based feature projector that contain learnable memory vectors to extract modality-shared features better. More importantly, during the model training, we calculate four kinds of similarity distributions (text-to-text, text-to-molecule, molecule-to-molecule, and molecule-to-text similarity distributions) for each instance, and then minimize the distance between these similarity distributions (namely second-order similarity losses) to enhance cross-modal alignment. Experimental results and analysis strongly demonstrate the effectiveness of our model. Particularly, our model achieves SOTA performance, outperforming the previously-reported best result by 6.4%.

==> tables/ablation.tex <==
\begin{table*}[ht]
    \centering
    \caption{Ablation study on the ChEBI-20 dataset at three levels: token-atom (TA), Multitoken-motif (MM), and sentence-molecule (SM). The bold part indicates the best performance. The results suggest that integrating three levels significantly improves performance in both text-molecule and molecule-text retrieval tasks. $\uparrow$ denotes that the higher is the better, while $\downarrow$ denotes that the lower is the better.}
    % \resizebox{1\textwidth}{!}{
    \begin{tabular}{ccc|cccc|cccc}
        \toprule
        \multicolumn{3}{c|}{\textbf{Level}} & \multicolumn{4}{c|}{\textbf{Text-Molecule Retrieval}} & \multicolumn{4}{c}{\textbf{Molecule-Text Retrieval}} \\
        \cmidrule(lr){1-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11}
        \textbf{TA} & \textbf{MM} & \textbf{SM} & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)} & \textbf{MRR($\uparrow$)} & \textbf{Mean Rank($\downarrow$)} & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)} & \textbf{MRR($\uparrow$)} & \textbf{Mean Rank($\downarrow$)} \\
        \midrule
        \cmark & \cmark & \cmark & \textbf{66.5\%} & \textbf{93.9\%} & \textbf{0.772} & \textbf{18.53} & \textbf{61.6\%} & \textbf{93.8\%} & \textbf{0.739} & \textbf{8.1} \\
        \midrule
        \cmark & \cmark &  & 57.4\% & 91.6\% & 0.700 & 26.74 & 38.4\% & 89.4\% & 0.552 & 12.87 \\
        \cmark &  & \cmark & 61.7\% & 92.5\% & 0.733 & 23.10 & 51.9\% & 91.3\% & 0.661 & 11.13 \\
         & \cmark & \cmark & 35.6\% & 81.8\% & 0.511 & 41.39 & 35.1\% & 80.8\% & 0.506 & 30.95 \\
        \midrule
         &  & \cmark & 24.1\% & 75.3\% & 0.401 & 42.28 & 21.8\% & 72.1\% & 0.377 & 30.86 \\
        & \cmark &  & 17.0\% & 55.0\% & 0.291 & 219.45 & 20.2\% & 56.3\% & 0.319 & 247.27 \\
        \cmark &  &  & 49.6\% & 89.1\% & 0.636 & 37.17 & 23.3\% & 71.6\% & 0.384 & 22.64 \\
        \bottomrule
    \end{tabular}
    % }
    \label{tab:ablation}
\end{table*}


==> tables/retrieval_chebi.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Performance on the ChEBI-20 dataset for text-molecule and molecule-text retrieval tasks. The bold part indicates the best performance. ORMA achieves leading performance in both retrieval tasks. $\uparrow$ denotes that the higher is the better, while $\downarrow$ denotes that the lower is the better. \textbf{$^\dag$: our reproduced results of Atomas-base and the other results are reported in the previous works.}}
    % \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{4}{c|}{\textbf{Text-Molecule Retrieval}} & \multicolumn{4}{c}{\textbf{Molecule-Text Retrieval}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)}
        & \textbf{MRR($\uparrow$)} & \textbf{Mean Rank($\downarrow$)} & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)} & \textbf{MRR($\uparrow$)} & \textbf{Mean Rank($\downarrow$)} \\ 
        \midrule
        MLP-Ensemble~\cite{text2mol2021edwards} & 29.4\% & 77.6\% & 0.452 & 20.78 & - & - & - & - \\
        GCN-Ensemble~\cite{text2mol2021edwards} & 29.4\% & 77.1\% & 0.447 & 28.77 & - & - & - & - \\
        All-Ensemble~\cite{text2mol2021edwards} & 34.4\% & 81.1\% & 0.499 & 20.21 & 25.2\% & 74.1\% & 0.408 & 21.77 \\
        \midrule
        MLP+Atten~\cite{text2mol2021edwards} & 22.8\% & 68.7\% & 0.375 & 30.37 & - & - & - & - \\
        MLP+FPG~\cite{fpg2000han} & 22.6\% & 68.6\% & 0.374 & 30.37 & - & - & - & - \\
        \midrule
        AMAN~\cite{adversarial2023zhao} & 49.4\% & 92.1\% & 0.647 & 16.01 & 46.6\% & 91.6\% & 0.625 & 16.50 \\
        Atomas-base$^\dag$~\cite{atomas2024zhang} & 50.1\% & 92.1\% & 0.653 & \textbf{14.49} & 45.6\% & 90.3\% & 0.614 & 15.12 \\
        \midrule
        \rowcolor{cyan!10}\textbf{ORMA (Ours)} & \textbf{66.5\%} & \textbf{93.9\%} & \textbf{0.772} & 18.53 & \textbf{61.6\%} & \textbf{93.8\%} & \textbf{0.739} & \textbf{8.10} \\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:retrieval_chebi20}
\end{table*}

% \begin{table*}[!ht]
%     \centering
%     \caption{Performance on the chEBI-20 dataset for text-molecule and molecule-text retrieval tasks. The bold part indicated the best performance. ORMA achieved leading performance in both retrieval tasks.}
%     % \resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{c|cccc|cccc}
%     \toprule
%         \multirow{2}{*}{\textbf{Models}} & \multicolumn{4}{c|}{\textbf{Text-Molecule Retrieval}} & \multicolumn{4}{c}{\textbf{Molecule-Text Retrieval}} \\
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9} & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)}
%         & \textbf{MRR($\uparrow$)} & \textbf{Mean Rank($\downarrow$)} & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)} & \textbf{MRR($\uparrow$)} & \textbf{Mean Rank($\downarrow$)} \\ 
%         \midrule
%         MLP-Ensemble~\cite{text2mol2021edwards} & 29.4\% & 77.6\% & 0.452 & 20.78 & - & - & - & - \\
%         GCN-Ensemble~\cite{text2mol2021edwards} & 29.4\% & 77.1\% & 0.447 & 28.77 & - & - & - & - \\
%         All-Ensemble~\cite{text2mol2021edwards} & 34.4\% & 81.1\% & 0.499 & 20.21 & 25.2\% & 74.1\% & 0.408 & 21.77 \\
%         \midrule
%         MLP+Atten~\cite{text2mol2021edwards} & 22.8\% & 68.7\% & 0.375 & 30.37 & - & - & - & - \\
%         MLP+FPG~\cite{fpg2000han} & 22.6\% & 68.6\% & 0.374 & 30.37 & - & - & - & - \\
%         \midrule
%         AMAN~\cite{adversarial2023zhao} & 49.4\% & 92.1\% & 0.647 & 16.01 & 46.6\% & 91.6\% & 0.625 & 16.50 \\
%         Atomas-base~\cite{atomas2024zhang} & 50.1\% & 92.1\% & 0.653 & \textbf{14.49} & 45.6\% & 90.3\% & 0.614 & 15.12 \\
%         \midrule
%         \rowcolor{cyan!10}\textbf{ORMA (Ours)} & \textbf{66.5\%} & \textbf{93.9\%} & \textbf{0.772} & 18.53 & \textbf{61.6\%} & \textbf{93.8\%} & \textbf{0.739} & \textbf{8.10} \\
%     \bottomrule
%     \end{tabular}
%     % }
%     \label{tab:retrieval_chebi20}
% \end{table*}



% 历史版本 Hits@1
% \begin{table*}[!ht]
%     \centering
%     \caption{}
%     % \resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{c|cccc|cccc}
%     \toprule
%         \multirow{2}{*}{\textbf{Methods}} & \multicolumn{4}{c|}{\textbf{Text-to-Molecule Retrieval}} & \multicolumn{4}{c}{\textbf{Molecule-to-Text Retrieval}} \\
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9} & \textbf{Mean Rank($\downarrow$)} & \textbf{MRR($\uparrow$)}
%         & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)} & \textbf{Mean Rank($\downarrow$)} & \textbf{MRR($\uparrow$)} & \textbf{Hits@1($\uparrow$)} & \textbf{Hits@10($\uparrow$)} \\ 
%         \midrule
%         MLP1 & 30.38 & 0.372 & 22.4\% & 68.6\% & 28.89 & 0.350 & 19.8\% & 66.9\% \\
%         MLP2 & 30.72 & 0.369 & 22.3\% & 68.0\% & - & - & - & - \\
%         MLP3 & 36.30 & 0.372 & 22.3\% & 67.9\% & - & - & - & - \\
%         \midrule
%         GCN1 & 42.28 & 0.366 & 21.7\% & 68.2\% & 42.28 & 0.366 & 21.7\% & 68.2\% \\
%         GCN2 & 41.90 & 0.371 & 22.3\% & 68.9\% & - & - & - & - \\
%         GCN3 & 39.11 & 0.366 & 22.3\% & 67.9\% & - & - & - & - \\
%         \midrule
%         MLP-Ensemble & 20.78 & 0.452 & 29.4\% & 77.6\% & - & - & - & - \\
%         GCN-Ensemble & 28.77 & 0.447 & 29.4\% & 77.1\% & - & - & - & - \\
%         All-Ensemble & 20.21 & 0.499 & 34.4\% & 81.1\% & 21.77 & 0.408 & 25.2\% & 74.1\% \\
%         \midrule
%         MLP1+Atten & 30.37 & 0.375 & 22.8\% & 68.7\% & - & - & - & - \\
%         MLP1+FPG & 30.37 & 0.374 & 22.6\% & 68.6\% & - & - & - & - \\
%         \midrule
%         AMAN & 16.01 & 0.647 & 49.4\% & 92.1\% & 16.50 & 0.625 & 46.6\% & 91.6\% \\
%         Atomas-base & 14.85 & 0.640 & 48.8\% & 83.5\% & 15.13 & 0.614 & 45.6\% & 82.1\% \\
%         \midrule
%         Ours & - & - & - & - & - & - & - & - \\
%     \bottomrule
%     \end{tabular}
%     % }
%     \label{tab:retrieval_chebi20}
% \end{table*}

==> tables/retrieval_pcdes.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Performance on the PCdes dataset for text-molecule and molecule-text retrieval tasks, distinguishing among zero-shot, finetuning and from-scratch. The bold part indicates the best performance. Our model ORMA, trained from scratch, significantly outperforms others in all metrics. $\uparrow$ denotes that the higher is the better.}
    % \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{4}{c|}{\textbf{Text-Molecule Retrieval}} & \multicolumn{4}{c}{\textbf{Molecule-Text Retrieval}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} & \textbf{R@1($\uparrow$)} & \textbf{R@5($\uparrow$)} & \textbf{R@10($\uparrow$)} & \textbf{MRR($\uparrow$)} & \textbf{R@1($\uparrow$)} & \textbf{R@5($\uparrow$)} & \textbf{R@10($\uparrow$)} & \textbf{MRR($\uparrow$)} \\ 
        \midrule
        \rowcolor{gray!20}\multicolumn{9}{l}{\textit{Pretrained Model + Zero-shot}} \\
        MoMu~\cite{momu2022su} & 4.9\% & 14.5\% & 20.7\% & 0.103 & 5.1\% & 12.8\% & 18.9\% & 0.099 \\
        MolCA~\cite{molca2023liu} & 35.1\% & 62.1\% & 69.8\% & 0.473 & 38.0\% & 66.8\% & 74.5\% & 0.508 \\
        MolFM~\cite{molfm2023luo} & 16.1\% & 30.7\% & 39.5\% & 0.236 & 13.9\% & 28.7\% & 36.2\% & 0.214 \\
        MoleculeSTM~\cite{moleculestm2023liu} & 35.8\% & - & - & - & 39.5\% & - & - & - \\
        Atomas-base~\cite{atomas2024zhang} & 39.1\% & 59.7\% & 66.6\% & 0.473 & 37.9\% & 59.2\% & 65.6\% & 0.478 \\
        Atomas-large~\cite{atomas2024zhang} & 49.1\% & 68.3\% & 73.2\% & 0.578 & 46.2\% & 66.0\% & 72.3\% & 0.555 \\
        \midrule
        \rowcolor{gray!20}\multicolumn{9}{l}{\textit{Pretrained Model + Finetuning}} \\
        SciBERT~\cite{scibert2019beltagy} & 16.3\% & 33.9\% & 42.6\% & 0.250 & 15.0\% & 34.1\% & 41.7\% & 0.239 \\
        KV-PLM~\cite{deep2022zeng} & 18.4\% & 37.2\% & 45.4\% & 0.274 & 16.6\% & 35.9\% & 44.8\% & 0.260 \\
        KV-PLM*~\cite{deep2022zeng} & 20.6\% & 37.9\% & 45.7\% & 0.292 & 19.3\% & 37.3\% & 45.3\% & 0.281 \\
        MoMu~\cite{momu2022su} & 24.5\% & 45.4\% & 53.8\% & 0.343 & 24.9\% & 44.9\% & 54.3\% & 0.345 \\
        MolFM~\cite{molfm2023luo} & 29.8\% & 50.5\% & 58.6\% & 0.396 & 29.4\% & 50.3\% & 58.5\% & 0.393 \\
        \midrule
        \rowcolor{gray!20}\multicolumn{9}{l}{\textit{From-scratch}} \\
        \rowcolor{cyan!10}\textbf{ORMA (Ours)} & \textbf{64.8\%} & \textbf{82.3\%} & \textbf{86.3\%} & \textbf{0.727} & \textbf{62.1\%} & \textbf{81.4\%} & \textbf{86.3\%} & \textbf{0.710} \\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:retrieval_pcdes}
\end{table*}

